Deep R-Learning for Continual Area Sweeping

Coverage path planning is a well-studied problem in robotics in which a robot must plan a path that passes through every point in a given area repeatedly, usually with a uniform frequency. To address the scenario in which some points need to be visited more frequently than others, this problem has been extended to non-uniform coverage planning. This paper considers the variant of non-uniform coverage in which the robot does not know the distribution of relevant events beforehand and must nevertheless learn to maximize the rate of detecting events of interest. This continual area sweeping problem has been previously formalized in a way that makes strong assumptions about the environment, and to date only a greedy approach has been proposed. We generalize the continual area sweeping formulation to include fewer environmental constraints, and propose a novel approach based on reinforcement learning in a Semi-Markov Decision Process. This approach is evaluated in an abstract simulation and in a high fidelity Gazebo simulation. These evaluations show significant improvement upon the existing approach in general settings, which is especially relevant in the growing area of service robotics.

==> related_work.tex <==
\section{Related Work}
% Compact stuff about semantic mapping, and expand about sweeping stuff Use Mazda's literature survey
Coverage path planning, also known as terrain coverage or sweeping, is a problem in which, given a map of an environment, the goal of agents traversing that map is to generate a path such that the the agent passes through the entire volume of the map \cite{choset2001coverage,gabriely2001spanning,Galceran:2013:SCP:2542686.2542724}. This approach is useful for a variety of applications where the robot must travel over the entire area, such as lawn mowing or vacuum cleaning. Significant work has also been done on sweeping in multi-robot settings, \cite{kurabayashi1996cooperative,zlot2002multi}, where the problem can be expressed efficiently as the path planning or traversal behavior of multiple robots.

Ahmadi and Stone [\citeyear{ahmadi2005continuous}] introduced the continual area sweeping problem as a specialization of this problem (and followed-up with a multi-robot case \cite{ahmadi2006multi}) where the goal of the agent is to provide greater coverage to areas where more activity occurs. Their goal is similar to that of the cleaning robot from above, but enabling it to autonomously focus on high-traffic areas where a greater amount of mess accumulates. The problem is modeled over a grid, where an event occurs in each grid cell according to a random distribution. They also present an initial approach to this problem; a greedy approach to minimizing the average time it takes to detect an event once it has occurred, which we refer to in this paper as \textsc{adt-greedy}. %We present an approach in this paper which attempts to learn an optimal policy over a similarly-defined grid.

The motivation for this work is to enable autonomous service robots to maintain a high degree of awareness of their environment. We approach this problem as one related to semantic mapping problems, of which there are a variety. Nuchter et al [\citeyear{nuchter20053d}] labeled detected terrain in 3D maps as belonging to entities such as floors or ceilings. Hart et al [\citeyear{hart2018prism}] incorporate room number information into their map so their robot can navigate to specific rooms. Mason et al [\citeyear{mason2012object}] use perceptual data to discuss objects in the scene. Important in their system is change detection, where semantics are updated when they have changed in the environment. Similarly, SOMA concentrates on the exploration of objects and change over time \cite{kunze-soma}. Robust, autonomous exploration of map data is possible through frontier-based exploration methods \cite{yamauchi1997frontier}, though we have not yet seen such a complete search expanded to semantic mapping. However, Jebari et al [\citeyear{jebari2011multi}] develop a stochastic method for autonomous exploration of an area in 2D using a Lidar unit, then scanning for objects using a pan-tilt camera. The present work is a step toward a continual scan of an area for the purpose of updating information in a semantic map. Our eventual goal is to excel in maintaining awareness of the scene, keeping an up-to-date semantic map by using RL to inform the robot of good exploration strategies that are likely to provide information updates.

Additionally, patrolling is a related problem that operates in a similar setting. Gatti [\citeyear{gatti2008game}] describes a game theoretic approach based on adversarial guard and robber agents that act strategically. Much of other work in this area is concerned with such an adversarial two player game scenario \cite{basilico2012patrolling,bovsansky2011computing}. However, in this work, we are not focused on adversarial games between players, as instead the motivation arises from service robot environments where events from tasks like cleaning or semantic mapping do not strategically appear in a way designed to counter detection.

%and provide an initial solution .

%However, these approaches aim to cover an entire spatial region and do not explicitly account for keeping up to date semantics which causes a lot of unnecessary re-exploration of semantically irrelevant areas.

 %However, they take a greedy approach to minimizing average detection time of events. This is in contrast with our approach, which is not greedy by virtue of learning the optimal policy.
%However, their approach assumes that the probabilities of events occurring in a region of the map are constant in time. This fails to capture important temporal dependencies. For example, a kitchen area would need to be visited around lunchtime, but is less important otherwise. Moreover, they take a greedy approach to minimizing average cost, and the problem is not modeled as a sequential decision making process. We aim to handle these limitations in our work, as we are not learning a greedy policy, and time is an important part of our state space. 
